From NoSQL Accumulo to NewSQL Graphulo: Design and Utility of Graph Algorithms inside a BigTable Database

Google BigTable's scale-out design for distributed key-value storage inspired a generation of NoSQL databases. Recently the NewSQL paradigm emerged in response to analytic workloads that demand distributed computation local to data storage. Many such analytics take the form of graph algorithms, a trend that motivated the GraphBLAS initiative to standardize a set of matrix math kernels for building graph algorithms. In this article we show how it is possible to implement the GraphBLAS kernels in a BigTable database by presenting the design of Graphulo, a library for executing graph algorithms inside the Apache Accumulo database. We detail the Graphulo implementation of two graph algorithms and conduct experiments comparing their performance to two main-memory matrix math systems. Our results shed insight into the conditions that determine when executing a graph algorithm is faster inside a database versus an external system---in short, that memory requirements and relative I/O are critical factors.

==> Makefile <==
# input file name.  This defines the name of the file you want to latex
# the make file will automatically look for INPUT.tex as the latex file
# and will look for a INPUT.bib file for the bibliography
INPUT=2016-HPEC-Graphulo-Graph-Algorithms
BIBFILE=10_bibliography
INC=3TrussAdjTime-20160526-114752.png GraphuloRate-20160526-114916.png JaccardTime-20160526-114916.png \
TwoTableOverview.png 01_introduction.tex 00_abstract.tex JaccardViz.png
#PS1='${debian_chroot:+($debian_chroot)}\[\033[01;32m\]\u@\h\[\033[00m\]:\[\033[01;34m\]\w\[\033[00m\]\$ '
#commands 
TEX=latex
PDFTEX=pdflatex
LYX=lyx
BIBTEX=bibtex
DVIPS=dvips -t letter
PS2PDF=ps2pdf14 -dPDFSETTINGS=/prepress

#extensions
DVIEXT=.dvi
PSEXT=.ps
TEXEXT=.tex
BIBEXT=.bib
LYXEXT=.lyx
PDFEXT=.pdf

default: pdf

dvi: latex bibtex latex2

latex: 
	$(TEX) $(INPUT)$(TEXEXT)

latex2:
	$(TEX) $(INPUT)$(TEXEXT)
	$(TEX) $(INPUT)$(TEXEXT)

pdflatex: 
	$(PDFTEX) $(INPUT)$(TEXEXT)

pdflatex2:
	$(PDFTEX) $(INPUT)$(TEXEXT)
	$(PDFTEX) $(INPUT)$(TEXEXT)

bibtex: $(BIBFILE)$(BIBEXT) 
	$(BIBTEX) $(INPUT)

ps: dvi
	$(DVIPS) -o $(INPUT)$(PSEXT) $(INPUT)$(DVIEXT)

pspdf: ps
	$(PS2PDF) $(INPUT)$(PSEXT)

pdf: pdflatex bibtex pdflatex2

gentex:
	$(LYX) --export latex $(INPUT)-lyx$(LYXEXT)

viewdvi:
	kdvi $(INPUT)$(DVIEXT)

view: kpdf

kpdf:
	okular $(INPUT)$(PDFEXT)

clean:
	rm -f $(INPUT)$(PSEXT)
	rm -f $(INPUT)$(DVIEXT) 
	rm -f *.aux *.bbl *.blg *.log *.toc *.fdb_latexmk *.fls	*.synctex.gz

cleaner: clean
	rm -f *~
	rm -f $(INPUT)$(PDFEXT)

tar:
	tar czvf $(INPUT).tar.gz Makefile $(INPUT).tex $(BIBFILE).bib $(INC)



==> l3docstrip.tex <==
%%
%% This is file `l3docstrip.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% l3docstrip.dtx  (with options: `program')
%% 
%% EXPERIMENTAL CODE
%% 
%% Do not distribute this file without also distributing the
%% source files specified above.
%% 
%% Do not distribute a modified version of this file.
%% 
%% File l3dosctrip.dtx Copyright (C) 2012 The LaTeX3 Project
%%
%% It may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License (LPPL), either version 1.3c of this
%% license or (at your option) any later version.  The latest version
%% of this license is in the file
%%
%%    http://www.latex-project.org/lppl.txt
%%
%% This file is part of the "l3kernel bundle" (The Work in LPPL)
%% and all files in that bundle must be distributed together.
%%
%% The released version of this bundle is available from CTAN.
%%
%% -----------------------------------------------------------------------
%%
%% The development version of the bundle can be found at
%%
%%    http://www.latex-project.org/svnroot/experimental/trunk/
%%
%% for those people who are interested.
%%
%%%%%%%%%%%
%% NOTE: %%
%%%%%%%%%%%
%%
%%   Snapshots taken from the repository represent work in progress and may
%%   not work or may contain conflicting material!  We therefore ask
%%   people _not_ to put them into distributions, archives, etc. without
%%   prior consultation with the LaTeX Project Team.
%%
%% -----------------------------------------------------------------------
%%
\def\ExplFileDate{2012/06/08}
\def\ExplFileName{l3docstrip}
\def\ExplFileVersion{3787}
\input docstrip %
\def\checkOption<#1{%
  \ifcase
    \ifx*#10\else \ifx/#11\else
    \ifx+#12\else \ifx-#13\else
    \ifx<#14\else \ifx @#15\else 6\fi\fi\fi\fi\fi\fi\relax
  \expandafter\starOption\or
  \expandafter\slashOption\or
  \expandafter\plusOption\or
  \expandafter\minusOption\or
  \expandafter\verbOption\or
  \expandafter\moduleOption\or
  \expandafter\doOption\fi
  #1%
}
\def\moduleOption @@=#1>#2\endLine{%
  \maybeMsg{<@@=#1>}%
  \prepareActiveModule{#1}%
}
\begingroup
  \catcode`\_ = 12 %
  \long\gdef\prepareActiveModule#1{%
    \ifx\relax#1\relax
       \let\replaceModuleInLine\empty
    \else
      \def\replaceModuleInLine{%
        \replaceAllIn\inLine{__@@}{__#1}%
        \replaceAllIn\inLine{_@@}{__#1}%
        \replaceAllIn\inLine{@@}{__#1}%
      }%
    \fi
  }
\endgroup
\let\replaceModuleInLine\empty
\long\def\replaceAllIn#1#2#3{%
  \long\def\tempa##1##2#2{%
    ##2\qMark\replaceAllInAuxIII#3##1%
  }%
  \edef#1{\expandafter\replaceAllInAuxI#1\qMark#2\qStop}%
}
\def\replaceAllInAuxI{%
  \expandafter\replaceAllInAuxII\tempa\replaceAllInAuxI\empty
}
\long\def\replaceAllInAuxII#1\qMark#2{#1}
\long\def\replaceAllInAuxIII#1\qStop{}
\def\normalLine#1\endLine{%
  \maybeMsg{.}%
  \def\inLine{#1}%
  \replaceModuleInLine
  \let\do\putline@do
  \activefiles
}
%% 
%%
%% End of file `l3docstrip.tex'.

